Generative Flows with Invertible Attentions

Flow-based generative models have shown an excellent ability to explicitly learn the probability density function of data via a sequence of invertible transformations. Yet, learning attentions in generative flows remains understudied, while it has made breakthroughs in other domains. To fill the gap, this paper introduces two types of invertible attention mechanisms, i.e., map-based and transformer-based attentions, for both unconditional and conditional generative flows. The key idea is to exploit a masked scheme of these two attentions to learn long-range data dependencies in the context of generative flows. The masked scheme allows for invertible attention modules with tractable Jacobian determinants, enabling its seamless integration at any positions of the flow-based models. The proposed attention mechanisms lead to more efficient generative flows, due to their capability of modeling the long-term data dependencies. Evaluation on multiple image synthesis tasks shows that the proposed attention flows result in efficient models and compare favorably against the state-of-the-art unconditional and conditional generative flows.

==> 08_references.tex <==
\begin{thebibliography}{10}\itemsep=-1pt

\bibitem{BehrmannGCDJ19}
Jens Behrmann, Will Grathwohl, Ricky T.~Q. Chen, David Duvenaud, and
  J{\"{o}}rn{-}Henrik Jacobsen.
\newblock Invertible residual networks.
\newblock In {\em ICML}, pages 573--582, 2019.

\bibitem{BreglerO94}
Christoph Bregler and Stephen~M. Omohundro.
\newblock Nonlinear image interpolation using manifold learning.
\newblock In {\em NIPS}, pages 973--980, 1994.

\bibitem{BrockDS19}
Andrew Brock, Jeff Donahue, and Karen Simonyan.
\newblock Large scale {GAN} training for high fidelity natural image synthesis.
\newblock In {\em ICLR}, 2019.

\bibitem{abs-1906-02735}
Ricky T.~Q. Chen, Jens Behrmann, David Duvenaud, and J{\"{o}}rn{-}Henrik
  Jacobsen.
\newblock Residual flows for invertible generative modeling.
\newblock In {\em NeurIPS}, pages 9913--9923, 2019.

\bibitem{0022KSDDSSA17}
Xi Chen, Diederik~P. Kingma, Tim Salimans, Yan Duan, Prafulla Dhariwal, John
  Schulman, Ilya Sutskever, and Pieter Abbeel.
\newblock Variational lossy autoencoder.
\newblock In {\em ICLR}, 2017.

\bibitem{ChenMRA18}
Xi Chen, Nikhil Mishra, Mostafa Rohaninejad, and Pieter Abbeel.
\newblock Pixelsnail: An improved autoregressive generative model.
\newblock In {\em ICML}, pages 864--872, 2018.

\bibitem{DielemanOS18}
Sander Dieleman, A{\"{a}}ron van~den Oord, and Karen Simonyan.
\newblock The challenge of realistic music generation: {M}odelling raw audio at
  scale.
\newblock In {\em NeurIPS}, pages 7989--7999, 2018.

\bibitem{DinhKB14}
Laurent Dinh, David Krueger, and Yoshua Bengio.
\newblock {NICE:} {N}on-linear independent components estimation.
\newblock In {\em ICLR Workshop}, 2015.

\bibitem{DinhSB17}
Laurent Dinh, Jascha Sohl{-}Dickstein, and Samy Bengio.
\newblock Density estimation using real {NVP}.
\newblock In {\em ICLR}, 2017.

\bibitem{domke2008killed}
Justin Domke, Alap Karapurkar, and Yiannis Aloimonos.
\newblock Who killed the directed model?
\newblock In {\em CVPR}, 2008.

\bibitem{GoodfellowPMXWOCB14}
Ian~J. Goodfellow, Jean Pouget{-}Abadie, Mehdi Mirza, Bing Xu, David
  Warde{-}Farley, Sherjil Ozair, Aaron~C. Courville, and Yoshua Bengio.
\newblock Generative adversarial nets.
\newblock In {\em NIPS}, pages 2672--2680, 2014.

\bibitem{Graves13}
Alex Graves.
\newblock Generating sequences with recurrent neural networks.
\newblock {\em arXiv:1308.0850}, 2013.

\bibitem{HeuselRUNH17}
Martin Heusel, Hubert Ramsauer, Thomas Unterthiner, Bernhard Nessler, and Sepp
  Hochreiter.
\newblock {GANs} trained by a two time-scale update rule converge to a local
  {N}ash equilibrium.
\newblock In {\em NeurIPS}, pages 6626--6637, 2017.

\bibitem{HoCSDA19}
Jonathan Ho, Xi Chen, Aravind Srinivas, Yan Duan, and Pieter Abbeel.
\newblock Flow++: Improving flow-based generative models with variational
  dequantization and architecture design.
\newblock In {\em ICML}, pages 2722--2730, 2019.

\bibitem{HochreiterS97}
Sepp Hochreiter and J{\"{u}}rgen Schmidhuber.
\newblock Long short-term memory.
\newblock {\em Neural Computation}, 9(8):1735--1780, 1997.

\bibitem{HoogeboomBW19}
Emiel Hoogeboom, Rianne van~den Berg, and Max Welling.
\newblock Emerging convolutions for generative normalizing flows.
\newblock In {\em ICML}, pages 2771--2780, 2019.

\bibitem{KalchbrennerESN18}
Nal Kalchbrenner, Erich Elsen, Karen Simonyan, Seb Noury, Norman Casagrande,
  Edward Lockhart, Florian Stimberg, A{\"{a}}ron van~den Oord, Sander Dieleman,
  and Koray Kavukcuoglu.
\newblock Efficient neural audio synthesis.
\newblock In {\em ICML}, pages 2410--2419, 2018.

\bibitem{KingmaD18}
Diederik~P. Kingma and Prafulla Dhariwal.
\newblock Glow: Generative flow with invertible 1x1 convolutions.
\newblock In {\em NeurIPS}, pages 10215--10224, 2018.

\bibitem{kingma2016improved}
Diederik~P. Kingma, Tim Salimans, Rafal Jozefowicz, Xi Chen, Ilya Sutskever,
  and Max Welling.
\newblock Improved variational inference with inverse autoregressive flow.
\newblock In {\em NIPS}, pages 4743--4751, 2016.

\bibitem{KingmaW13}
Diederik~P. Kingma and Max Welling.
\newblock Auto-encoding variational {B}ayes.
\newblock In {\em ICLR}, 2014.

\bibitem{krizhevsky2009learning}
Alex Krizhevsky, Geoffrey Hinton, et~al.
\newblock Learning multiple layers of features from tiny images.
\newblock Technical report, U. of Toronto, 2009.

\bibitem{lecun1998gradient}
Yann LeCun, L{\'e}on Bottou, Yoshua Bengio, Patrick Haffner, et~al.
\newblock Gradient-based learning applied to document recognition.
\newblock {\em Proc. IEEE}, 86(11):2278--2324, 1998.

\bibitem{MenickK19}
Jacob Menick and Nal Kalchbrenner.
\newblock Generating high fidelity images with subscale pixel networks and
  multidimensional upscaling.
\newblock In {\em ICLR}, 2019.

\bibitem{OstrovskiDM18}
Georg Ostrovski, Will Dabney, and R{\'{e}}mi Munos.
\newblock Autoregressive quantile networks for generative modeling.
\newblock In {\em ICML}, pages 3936--3945, 2018.

\bibitem{PapamakariosMP17}
George Papamakarios, Iain Murray, and Theo Pavlakou.
\newblock Masked autoregressive flow for density estimation.
\newblock In {\em NeurIPS}, pages 2338--2347, 2017.

\bibitem{ParmarVUKSKT18}
Niki Parmar, Ashish Vaswani, Jakob Uszkoreit, Lukasz Kaiser, Noam Shazeer,
  Alexander Ku, and Dustin Tran.
\newblock Image transformer.
\newblock In {\em ICML}, pages 4055--4064, 2018.

\bibitem{RadfordMC15}
Alec Radford, Luke Metz, and Soumith Chintala.
\newblock Unsupervised representation learning with deep convolutional
  generative adversarial networks.
\newblock In {\em ICLR}, 2016.

\bibitem{abs-1906-00446}
Ali Razavi, A{\"{a}}ron van~den Oord, and Oriol Vinyals.
\newblock Generating diverse high-fidelity images with {VQ-VAE-2}.
\newblock In {\em NeurIPS}, pages 14837--14847, 2019.

\bibitem{ReedOKCWCBF17}
Scott~E. Reed, A{\"{a}}ron van~den Oord, Nal Kalchbrenner, Sergio~Gomez
  Colmenarejo, Ziyu Wang, Yutian Chen, Dan Belov, and Nando de Freitas.
\newblock Parallel multiscale autoregressive density estimation.
\newblock In {\em ICML}, pages 2912--2921, 2017.

\bibitem{RezendeMW14}
Danilo~Jimenez Rezende, Shakir Mohamed, and Daan Wierstra.
\newblock Stochastic backpropagation and approximate inference in deep
  generative models.
\newblock In {\em ICML}, pages 1278--1286, 2014.

\bibitem{Russakovsky:2015:ILS}
Olga Russakovsky, Jia Deng, Hao Su, Jonathan Krause, Sanjeev Satheesh, Sean Ma,
  Zhiheng Huang, Andrej Karpathy, Aditya Khosla, Michael Bernstein,
  Alexander~C. Berg, and Li Fei-Fei.
\newblock {ImageNet} large scale visual recognition challenge.
\newblock {\em International Journal of Computer Vision}, 115(13):211--252,
  2015.

\bibitem{SalimansGZCRCC16}
Tim Salimans, Ian~J. Goodfellow, Wojciech Zaremba, Vicki Cheung, Alec Radford,
  and Xi Chen.
\newblock Improved techniques for training {GANs}.
\newblock In {\em NIPS}, pages 2234--2242, 2016.

\bibitem{SalimansK0K17}
Tim Salimans, Andrej Karpathy, Xi Chen, and Diederik~P. Kingma.
\newblock {PixelCNN++}: {I}mproving the {PixelCNN} with discretized logistic
  mixture likelihood and other modifications.
\newblock In {\em ICLR}, 2017.

\bibitem{ShiGL0YWW17}
Xingjian Shi, Zhihan Gao, Leonard Lausen, Hao Wang, Dit{-}Yan Yeung, Wai{-}Kin
  Wong, and Wang{-}chun Woo.
\newblock Deep learning for precipitation nowcasting: {A} benchmark and a new
  model.
\newblock In {\em NeurIPS}, pages 5617--5627, 2017.

\bibitem{TheisOB15}
Lucas Theis, A{\"{a}}ron van~den Oord, and Matthias Bethge.
\newblock A note on the evaluation of generative models.
\newblock In {\em ICLR}, 2016.

\bibitem{TomczakW18}
Jakub~M. Tomczak and Max Welling.
\newblock {VAE} with a {VampPrior}.
\newblock In {\em AISTATS}, pages 1214--1223, 2018.

\bibitem{OordKEKVG16}
A{\"{a}}ron van~den Oord, Nal Kalchbrenner, Lasse Espeholt, Koray Kavukcuoglu,
  Oriol Vinyals, and Alex Graves.
\newblock Conditional image generation with {PixelCNN} decoders.
\newblock In {\em NIPS}, pages 4790--4798, 2016.

\bibitem{OordKK16}
A{\"{a}}ron van~den Oord, Nal Kalchbrenner, and Koray Kavukcuoglu.
\newblock Pixel recurrent neural networks.
\newblock In {\em ICML}, pages 1747--1756, 2016.

\bibitem{OordLBSVKDLCSCG18}
A{\"{a}}ron van~den Oord, Yazhe Li, Igor Babuschkin, Karen Simonyan, Oriol
  Vinyals, Koray Kavukcuoglu, George van~den Driessche, Edward Lockhart,
  Luis~C. Cobo, Florian Stimberg, Norman Casagrande, Dominik Grewe, Seb Noury,
  Sander Dieleman, Erich Elsen, Nal Kalchbrenner, Heiga Zen, Alex Graves, Helen
  King, Tom Walters, Dan Belov, and Demis Hassabis.
\newblock Parallel {WaveNet}: {F}ast high-fidelity speech synthesis.
\newblock In {\em ICML}, pages 3918--3926, 2018.

\bibitem{WeiGL0W18}
Xiang Wei, Boqing Gong, Zixia Liu, Wei Lu, and Liqiang Wang.
\newblock Improving the improved training of {W}asserstein {GANs}: {A}
  consistency term and its dual effect.
\newblock In {\em ICLR}, 2018.

\bibitem{ZieglerR19}
Zachary~M. Ziegler and Alexander~M. Rush.
\newblock Latent normalizing flows for discrete sequences.
\newblock In {\em ICML}, pages 7673--7682, 2019.

\end{thebibliography}
